Measuring What Matters in the Age of AI: The Research Software Metrics Landscape

Research software now serves as a primary instrument of science, but the methods the community uses to judge its quality, sustainability, reuse, and impact remain scattered across software engineering, open science, FAIR software, citation, and research-assessment literature. AI-assisted development sharpens the problem: code can be produced at rates that outpace human review capacity, provenance and attribution are harder to track, scholarly credit systems cannot keep pace, and existing metrics inherit assumptions about how research software gets developed that may no longer apply. To aid in navigating these challenges, we present a focused landscape synthesis of research software metrics based on 49 substantive references, organizing the recurring metrics into eight families described by data source, claimed construct, evidence of validity, automation potential, and susceptibility to misuse. Many widely cited research software metrics serve as partial signals but make weak standalone measures of scientific impact. The AI era opens or widens gaps around provenance, maintainability of generated code, reviewer effort, model and data dependencies, reuse and community-health signal inflation, and credit for human labor that AI does not perform. We argue for responsible, contextual, mixed-method use of research software metrics, and offer decision guidance for Research Software Engineers (RSEs), principal investigators, institutions, and funders selecting metrics that support better software, fairer credit, and more trustworthy science. All findings rest on the 49-reference focused review; a reproducible search-and-triage protocol and a 727-record triaged corpus accompany the paper as a transparency artifact for a future full systematic mapping study.

==> connection-statement.tex <==

This submission connects directly to the mission, goals, and interests of the US-RSE community by addressing how research software contributions are recognized, evaluated, sustained, and communicated. Research Software Engineers (RSEs) often create impact through activities that are difficult to capture in traditional scholarly metrics, including maintenance, code review, testing, documentation, user support, mentoring, and community building. By mapping the research software metrics landscape, this paper offers a shared vocabulary, a structured view of the eight recurring metric families it identifies, and decision guidance that can help RSEs, principal investigators, institutions, and funders discuss software quality, sustainability, reuse, and impact more clearly.
In the context of USRSE'26's theme, ``Advancing Science in the Age of AI,'' this paper argues that responsible research software metrics are critical infrastructure for trustworthy, sustainable, and equitable AI-era science. As AI-assisted development changes the economics of producing research code, the community's need for evidence about reliability, maintainability, provenance, credit, and stewardship grows rather than shrinks. The proposed landscape and research agenda aim to help the US-RSE community lead, rather than react to, that change.


==> figures/maturity-map.tex <==
\begin{figure}[!t]
\centering
\begin{tikzpicture}[
    every node/.style={font=\footnotesize},
    family/.style={
        circle, draw=takeawayBorder, fill=stageScreen!50, line width=0.5pt,
        minimum size=4mm, inner sep=0pt
    },
    flabel/.style={
        font=\scriptsize, align=center
    },
    axis/.style={
        -{Latex[length=1.4mm]}, semithick, draw=black!70
    },
    qlabel/.style={
        font=\scriptsize\itshape\color{black!55},
        align=center
    }
]

\def\W{7.6}
\def\H{5.6}

\fill[stageIncl!30] (0,\H/2) rectangle (\W/2,\H);
\fill[stageElig!35] (\W/2,\H/2) rectangle (\W,\H);
\fill[stageId!22]   (0,0)      rectangle (\W/2,\H/2);
\fill[stageScreen!22] (\W/2,0) rectangle (\W,\H/2);

\node[qlabel, anchor=north west] at (0.15,\H-0.15) {Early but\\AI-aware};
\node[qlabel, anchor=north east] at (\W-0.15,\H-0.15) {Mature \&\\AI-robust};
\node[qlabel, anchor=south west] at (0.15,0.15) {Early \&\\AI-vulnerable};
\node[qlabel, anchor=south east] at (\W-0.15,0.15) {Mature but\\AI-vulnerable};

\draw[axis] (0,0) -- (\W+0.3,0);
\draw[axis] (0,0) -- (0,\H+0.3);

\node[font=\scriptsize, anchor=north] at (\W/2,-0.05) {Validation maturity $\rightarrow$};
\node[font=\scriptsize, anchor=south, rotate=90] at (-0.15,\H/2) {AI-era robustness $\rightarrow$};



\node[family] (sq)  at (6.4,3.7) {};
\node[flabel, above=0.5mm of sq] {Software\\quality};

\node[family] (fair) at (5.4,3.3) {};
\node[flabel, below=0.5mm of fair] {FAIR \&\\reproducibility};

\node[family] (sus) at (4.2,3.0) {};
\node[flabel, right=0.5mm of sus] {Sustainability};

\node[family] (sec) at (3.0,2.6) {};
\node[flabel, above=0.5mm of sec] {Security \&\\supply chain};

\node[family] (env) at (1.8,1.9) {};
\node[flabel, right=0.5mm of env] {Environmental\\\& performance};

\node[family] (reuse) at (5.7,1.5) {};
\node[flabel, right=0.5mm of reuse] {Reuse \&\\adoption};

\node[family] (cred) at (3.7,0.9) {};
\node[flabel, right=0.5mm of cred] {Credit \&\\attribution};

\node[family] (ch) at (1.4,3.7) {};
\node[flabel, above=0.5mm of ch] {Community\\health};

\end{tikzpicture}
\caption{Metric Maturity Map. Each family is positioned by validation maturity ($x$) and robustness to AI-era pressures ($y$). Lower-left needs protocol changes most urgently; upper-right is best validated against current concerns.}
\label{fig:maturity}
\end{figure}

